Dynamic Logic with Parallel Operator for Verifying Communication Protocols

In this paper, we present a dynamic logic with parallel operators for the formal verification of authenticity and safety properties of cryptographic protocols. The logic incorporates communication actions and is specifically designed to reason about protocol executions in adversarial environments. We extend an existing dynamic logic with parallel operators by introducing concepts derived from the Dolev-Yao intruder model. As the underlying logic is completely axiomatizable, we obtain a complete axiomatization for the extended system. Furthermore, we develop a tableau calculus for the proposed logic and prove its termination, soundness, and completeness.

==> eptcsdata.tex <==
\providecommand{\firstpage}{55}
\providecommand{\publicationstatus}{V. de Paiva; T.A. de Lima (Eds.): 21st International Symposium\\ on Logical and Semantic Frameworks, with Applications (LSFA 2026)\\
EPTCS 449, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.449.4}{10.4204/EPTCS.449.4}}
\pdfoutput=1

